Entropy-aware non-oscillatory high-order finite volume methods using the Dafermos entropy rate criterion

Finite volume methods are popular tools for solving time-dependent partial differential equations, especially hyperbolic conservation laws. Over the past 40 years a popular way of enlarging their robustness was the enforcement of global or local entropy inequalities. This work focuses on a different entropy criterion proposed by Dafermos almost 50 years ago, stating that the weak solution should be selected that dissipates a selected entropy with the highest possible speed. We show that this entropy rate criterion can be used in a numerical setting if it is combined with the theory of optimal recovery. To date, this criterion has only seen limited use in Finite-Volume schemes and to the authors knowledge this work is the first in which this criterion is applied to a Finite-Volume scheme whose accuracy is based on reconstruction from mean values. This leads to a new family of schemes based on reconstruction providing an alternative to the popular ENO and WENO schemes.

==> 4_systems.tex <==
\section{Extensions to systems} 
\label{sec:systems} 


\subsection{Some examples} 

\begin{itemize}
    \item Shallow water equations
    \item Euler' equations 
    \item MHD equations
\end{itemize}

==> mycommands_sp.tex <==

\usepackage[english]{babel}
\usepackage{amsmath}
\usepackage{lineno}
\usepackage{caption}
\captionsetup{compatibility=false}
\usepackage{comment}
\usepackage{subcaption}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{mathptmx} 
\usepackage{xcolor}
\usepackage{tikz}
\usetikzlibrary{positioning}
\usepackage[square,numbers,sort]{natbib}
\usepackage{dsfont}
\usepackage{hyperref}

\renewcommand{\arraystretch}{1.4}
\smartqed


% notation and commands
\newcommand{\derive}[2] {{\frac{\partial {#1} }{\partial {#2}}}}
\newcommand{\derd}[2] {{\frac{\vd #1 }{\vd #2}}}
\newcommand{\diff}[2] {\varDelta_{#2} #1}

\newcommand{\lap}[2] {\nabla_{#2} #1}
\newcommand{\T}{\mathcal T}
\newcommand{\SubT}{\mathcal S}
\newcommand{\includepgf}[2]{\resizebox{#1}{!}{\input{#2}}}
\newcommand{\sd}[0]{\Omega \times \T}
\newcommand{\R}[0]{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\of}[1]{\left (#1 \right)}
\newcommand{\abs}[1]{\left | #1\right| }
\newcommand{\mabs}[1] {\,| #1 |}
\newcommand{\norm}[1]{\left \|#1  \right \|}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\set}[2]{ \{ #1 ~|~ #2\}}
\newcommand{\sset}[1]{ \{ #1\}}
\newcommand{\rest}[0]{|}
\newcommand{\Leb}{\mathrm{L}}
\newcommand{\inner}{\overset{\circ}}
\DeclareMathOperator{\convh}{conv}
\DeclareMathOperator{\ran}{ran}
\newcommand{\vd}{ \mathrm{d}}
\newcommand{\intd}{\,\mathrm{d}}
\newcommand{\lo}{\mathrm{LO}}
\newcommand{\ho}{\mathrm{HO}}
\newcommand{\te}{\mathrm{T, E}}
\newcommand{\refs}{\mathrm{ref}}
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\phi}{\varphi}
\newcommand{\skp}[2]{\left \langle {#1}, {#2} \right \rangle}
\newcommand{\bskp}[2]{\left [ {#1}, {#2} \right ]}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\bigO}{\mathcal{O}}
\DeclareMathOperator{\One}{\mathds{1}}
\DeclareMathOperator{\lspan}{span}
\DeclareMathOperator{\op}{\mathbb{P}}
\DeclareMathOperator{\ip}{\mathbb{I}}
\DeclareMathOperator{\ev}{\derive{U}{u}}
\newcommand{\NQ}[2]{\begin{tikzpicture}[baseline=-5.0pt, scale=0.2]
		\draw[line width=0.4mm](-1, -2) -- (-0.75, -2) node [anchor=west]{$\scriptstyle #1$} -- (-0.5, -2) -- (0.5, 2) -- (0.75, 2) node [anchor=west]{$\scriptstyle #2$} -- (1, 2);
\end{tikzpicture}}
\newcommand{\numd}{\begin{tikzpicture}[scale=0.15]
		\draw[line width=0.3mm] (1, 2.5)--(1, 0)--(0,0)--(0, 1)--(1,1);
	\end{tikzpicture}~}
\newcommand{\rskp}[2]{\left(#1\middle)\cdot\middle(#2\right)}
\newcommand{\drskp}[2]{#1 \cdot #2}
\DeclareMathOperator{\ch}{ch}
% theorems

%\theoremstyle{definition}
%\newtheorem{definition}{Definition}
%\theoremstyle{theorem}
%\newtheorem{lemma}{Lemma}
%\theoremstyle{remark}
%\newtheorem{example}{Example}
%\newtheorem{numexp}{Numerical Experiment}
%\theoremstyle{theorem}
%\newtheorem{theorem}{Theorem}
%\newtheorem{remark}{Remark}
%\newtheorem*{note}{Note}
%\newtheorem{corollary}{corollary}
\spnewtheorem{numexp}{Numerical Experiment}{\bf}{\it}
% WIP commands
\newcommand{\todo}[1]{{\color{red}#1}}
